From Traces to Agentic Worlds: Agentic Language World Models for Interactive Environment Simulation

Realistic environment replicas are increasingly valuable for training and evaluating LLM agents, yet the original systems may be inaccessible or impractical to reproduce. We explore agentic language world modeling: rather than rebuilding an executable environment, a world model agent serves as the environment for a task agent and supports faithful and stateful simulation. We instantiate this paradigm with Trace2Env, a learning-free framework for settings where the original system is unavailable but historical interaction traces remain accessible. Trace2Env reconstructs these traces into a reusable environment worldbook containing environment schemas, grounded evidence, and induced behavioral knowledge. At runtime, the world model agent actively consults the worldbook together with persistent episodic state to infer each action's observation and lasting state effects. Across nine environments, Trace2Env improves both next-observation fidelity and long-horizon interaction consistency over conventional prompt-based LWMs. In multi-turn interaction, task agent actions generated against Trace2Env remain valid more often when replayed in the real environment, indicating that its simulated dynamics better preserve the consequences of earlier actions across successive turns. These results establish agentic language world modeling as an alternative direction for building realistic environment replicas without reconstructing the original executable system.

==> components.tex <==
% Optional visual components for personalpaper.

\RequirePackage[ruled]{algorithm2e}
\RequirePackage{listings}
\RequirePackage{cleveref}
\RequirePackage{soul}
\tcbuselibrary{listings}

\RestyleAlgo{ruled}
\SetKwInput{Input}{Input}
\SetKwInput{Output}{Output}
\SetKwComment{Comment}{$\triangleright$\ }{}
\SetAlgoLined
\SetAlgoCaptionSeparator{\ \textcolor{ppaccent}{|}\ }
\SetAlCapNameFnt{\small\bfseries\color{ppnavy}}
\SetAlCapFnt{\small}
\DontPrintSemicolon

\newcounter{ppalgorithm}
\newenvironment{ppalgorithm}[1]{%
  \refstepcounter{ppalgorithm}%
  \begin{tcolorbox}[
    enhanced,
    breakable,
    colback=ppsoftblue!38!white,
    colframe=ppaccent!68!ppnavy,
    arc=1mm,
    boxrule=.45pt,
    top=1.1mm,
    bottom=1mm,
    left=1.2mm,
    right=1.2mm,
    before skip=8pt,
    after skip=8pt
  ]%
  {\small\bfseries\textcolor{ppnavy}{Algorithm~\theppalgorithm}\ \textcolor{ppaccent}{|}\ #1\par}%
  \vskip3pt
}{%
  \end{tcolorbox}%
}
\newcommand{\alginput}[1]{\noindent\textbf{Input:} #1\par}
\newcommand{\algoutput}[1]{\noindent\textbf{Output:} #1\par}
\newcommand{\algstep}[1]{%
  \par\noindent
  \hangindent=1.35em\hangafter=1
  \makebox[1.35em][l]{\textcolor{ppaccent}{\small$\triangleright$}}#1\par
}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\tcolorboxenvironment{theorem}{
  colback=ppsoftblue,
  colframe=ppnavy!70,
  arc=1mm,
  boxrule=.5pt,
  top=.7mm,
  bottom=.7mm,
  left=1mm,
  right=1mm,
  before skip=6pt,
  after skip=6pt
}

\tcolorboxenvironment{proposition}{
  colback=ppsoftblue,
  colframe=ppnavy!60,
  arc=1mm,
  boxrule=.5pt,
  top=.7mm,
  bottom=.7mm,
  left=1mm,
  right=1mm,
  before skip=6pt,
  after skip=6pt
}

\tcolorboxenvironment{definition}{
  colback=ppabsbg,
  colframe=ppaccent!70!black,
  arc=1mm,
  boxrule=.5pt,
  top=.7mm,
  bottom=.7mm,
  left=1mm,
  right=1mm,
  before skip=6pt,
  after skip=6pt
}

\tcolorboxenvironment{remark}{
  colback=ppsoftgray,
  colframe=ppmuted!70,
  arc=1mm,
  boxrule=.45pt,
  top=.7mm,
  bottom=.7mm,
  left=1mm,
  right=1mm,
  before skip=6pt,
  after skip=6pt
}

\tcolorboxenvironment{proof}{
  enhanced,
  breakable,
  colback=ppsoftblue!35!white,
  colframe=ppaccent!65!ppnavy,
  arc=1mm,
  boxrule=.4pt,
  top=.7mm,
  bottom=.7mm,
  left=1mm,
  right=1mm,
  before skip=6pt,
  after skip=8pt
}

\newtcolorbox{takeawaybox}[1][Takeaway]{
  enhanced,
  breakable,
  title=#1,
  colback=ppabsbg,
  colframe=ppnavy,
  fonttitle=\bfseries\small,
  coltitle=white,
  colbacktitle=ppnavy,
  attach boxed title to top left={xshift=2.5mm,yshift=-2.5mm},
  boxed title style={rounded corners, size=small, colframe=ppnavy, colback=ppnavy},
  arc=2mm,
  width=\linewidth
}

\newtcolorbox{highlightbox}[1][Highlight]{
  enhanced,
  breakable,
  title=#1,
  colback=ppsoftblue,
  colframe=ppaccent!80!black,
  fonttitle=\bfseries\small,
  coltitle=white,
  colbacktitle=ppaccent!80!black,
  attach boxed title to top left={xshift=2.5mm,yshift=-2.5mm},
  boxed title style={rounded corners, size=small, colframe=ppaccent!80!black, colback=ppaccent!80!black},
  arc=2mm,
  width=\linewidth
}

\definecolor{pppromptamber}{HTML}{B7791F}
\definecolor{pppromptblue}{HTML}{315F9D}
\definecolor{pppromptgreen}{HTML}{2F7D6D}
\definecolor{pppromptpurple}{HTML}{6B5CA5}
\definecolor{pppromptred}{HTML}{A23A34}
\definecolor{pppromptgray}{HTML}{69727D}
\definecolor{ppprompthl}{HTML}{FFE8A3}

\tcbset{
  pppromptbase/.style={
    enhanced,
    breakable,
    fonttitle=\bfseries\small,
    coltitle=white,
    attach boxed title to top left={xshift=2.5mm,yshift=-2.5mm},
    width=\linewidth,
    arc=2mm,
    boxrule=.55pt,
    top=2.8mm,
    bottom=1.2mm,
    left=1.2mm,
    right=1.2mm,
    before skip=8pt,
    after skip=8pt,
    fontupper=\small
  },
  promptbox/.style={
    pppromptbase,
    colback=pppromptamber!8,
    colframe=pppromptamber!80!black,
    colbacktitle=pppromptamber!80!black,
    boxed title style={rounded corners, size=small, boxrule=.4pt, colframe=pppromptamber!80!black, colback=pppromptamber!80!black}
  },
  promptboxblue/.style={
    pppromptbase,
    colback=pppromptblue!7,
    colframe=pppromptblue!80!black,
    colbacktitle=pppromptblue!80!black,
    boxed title style={rounded corners, size=small, boxrule=.4pt, colframe=pppromptblue!80!black, colback=pppromptblue!80!black}
  },
  promptboxgreen/.style={
    pppromptbase,
    colback=pppromptgreen!8,
    colframe=pppromptgreen!75!black,
    colbacktitle=pppromptgreen!75!black,
    boxed title style={rounded corners, size=small, boxrule=.4pt, colframe=pppromptgreen!75!black, colback=pppromptgreen!75!black}
  },
  promptboxpurple/.style={
    pppromptbase,
    colback=pppromptpurple!8,
    colframe=pppromptpurple!78!black,
    colbacktitle=pppromptpurple!78!black,
    boxed title style={rounded corners, size=small, boxrule=.4pt, colframe=pppromptpurple!78!black, colback=pppromptpurple!78!black}
  },
  promptboxred/.style={
    pppromptbase,
    colback=pppromptred!6,
    colframe=pppromptred!85!black,
    colbacktitle=pppromptred!85!black,
    boxed title style={rounded corners, size=small, boxrule=.4pt, colframe=pppromptred!85!black, colback=pppromptred!85!black}
  },
  promptboxgray/.style={
    pppromptbase,
    colback=ppsoftgray,
    colframe=pppromptgray!78!black,
    colbacktitle=pppromptgray!78!black,
    boxed title style={rounded corners, size=small, boxrule=.4pt, colframe=pppromptgray!78!black, colback=pppromptgray!78!black}
  }
}

\newcommand{\promptfield}[1]{\textbf{\textsc{#1}}}
\newcommand{\promptplaceholder}[1]{\texttt{\textless\detokenize{#1}\textgreater}}
\newcommand{\prompthl}[1]{\begingroup\sethlcolor{ppprompthl}\hl{#1}\endgroup}

\newtcblisting{promptlisting}[2][promptbox]{
  #1,
  title={#2},
  listing only,
  listing engine=listings,
  listing options={
    basicstyle=\ttfamily\scriptsize,
    breaklines=true,
    columns=fullflexible,
    keepspaces=true,
    showstringspaces=false
  }
}

\newcommand{\cmark}{\textcolor{ppgood}{\ding{51}}}
\newcommand{\xmark}{\textcolor{ppbad}{\ding{55}}}
\newcommand{\best}[1]{\cellcolor{ppaccent!18}\textbf{#1}}
\newcommand{\second}[1]{\cellcolor{ppsoftblue}\underline{#1}}
\newcommand{\gain}[1]{\textcolor{ppgood}{+#1}}
\newcommand{\loss}[1]{\textcolor{ppbad}{-#1}}

\lstdefinestyle{python}{
  language=Python,
  basicstyle=\ttfamily\small,
  keywordstyle=\color{pplink}\bfseries,
  stringstyle=\color{ppgood!80!black},
  commentstyle=\color{ppmuted}\itshape,
  showstringspaces=false,
  numbers=left,
  numberstyle=\tiny\color{ppmuted},
  stepnumber=1,
  numbersep=6pt,
  frame=single,
  rulecolor=\color{ppnavy!40},
  backgroundcolor=\color{ppsoftgray},
  breaklines=true,
  columns=fullflexible,
  keepspaces=true
}

\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{remark}{Remark}{Remarks}
\crefname{ppalgorithm}{Algorithm}{Algorithms}
\Crefname{ppalgorithm}{Algorithm}{Algorithms}
\crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefname{lstlisting}{Listing}{Listings}
\Crefname{lstlisting}{Listing}{Listings}





% ----------------------------------------------------------------------
% Custom link display text
% ----------------------------------------------------------------------

\newcommand{\projectlinktext}{Project}
\newcommand{\codelinktext}{Code}
\newcommand{\modellinktext}{Models}

% First argument: destination URL
% Second argument: display text in the PDF
\newcommand{\setprojectlink}[2]{%
  \projecturl{#1}%
  \renewcommand{\projectlinktext}{#2}%
}

\newcommand{\setcodelink}[2]{%
  \codeurl{#1}%
  \renewcommand{\codelinktext}{#2}%
}

\newcommand{\setmodellink}[2]{%
  \modelurl{#1}%
  \renewcommand{\modellinktext}{#2}%
}

\makeatletter

% ----------------------------------------------------------------------
% Unnumbered contact footnote
% ----------------------------------------------------------------------

% Remove the original contact line from the title block
\renewcommand{\pp@contactline}{}

% Remove the footnote marker and its reserved indentation
\newcommand{\pp@plainfootnotetext}[1]{\noindent #1}

% Place the contact email at the bottom of the first page
\g@addto@macro\maketitle{%
  \if\relax\the\correspondingauthor\relax
  \else
    \begingroup
      \renewcommand{\thefootnote}{}%
      \let\@makefntext\pp@plainfootnotetext
      \footnotetext[0]{%
        \textit{Corresponding author(s):}
        \href{mailto:\the\correspondingauthor}{\the\correspondingauthor}%
      }%
    \endgroup
  \fi
}

% ----------------------------------------------------------------------
% Center the links and use their custom display text
% ----------------------------------------------------------------------

\renewcommand{\pp@linkline}{%
  \begingroup
  \centering
  \if\relax\the\projecturl\relax\else
    {\linkfont \projectlinkicon\
      \href{\the\projecturl}{\projectlinktext}}\quad\quad\quad\quad
  \fi
  \if\relax\the\codeurl\relax\else
    {\linkfont \faGithub\
      \href{\the\codeurl}{\codelinktext}}\quad\quad\quad\quad
  \fi
  \if\relax\the\modelurl\relax\else
    {\linkfont \modellinkicon\
      \href{\the\modelurl}{\modellinktext}}%
  \fi
  \par
  \endgroup
}

\renewcommand{\pp@linkline}{%
  \begingroup
  \raggedright
  \if\relax\the\codeurl\relax\else
    {\fontsize{10pt}{10pt}\selectfont
      \faGithub\ 
      Code: \href{\the\codeurl}{\the\codeurl}%
    }%
  \fi
  \par
  \endgroup
}

\makeatother

% ----------------------------------------------------------------------
% Link destinations, display text, and contact email
% ----------------------------------------------------------------------

% \setprojectlink{https://example.com/project}{Project Website}
% \setcodelink{https://github.com/ViktorAxelsen/MemPilot}{GitHub Repository}
% \setmodellink{https://example.com/models}{Model Checkpoints}

% \correspondingauthor{wazhz14@gmail.com}
